On the Security of Semi Device Independent QKD protocols

While fully device-independent security in (BB84-like) prepare and measure Quantum Key Distribution (QKD) is impossible, it can be guaranteed against individual attacks in a semi device-independent (SDI) scenario, wherein no assumptions are made on the characteristics of the hardware used are made except for an upper bound on the the dimension of the communicated system. Studying security under such minimal assumptions is especially relevant in the context of the recent {\it quantum hacking} attacks wherein the eavesdroppers can not only construct the devices used by the communicating parties but are also able to remotely alter their behavior. In this work we study the security of a SDIQKD protocol based on the prepare and measure quantum implementation of a well-known cryptographic primitive, the Random Access Code (RAC). We consider imperfect detectors and establish the critical values of the security parameters (the observed success probability of the RAC and the detection efficiency) required for guaranteeing security against eavesdroppers with and without quantum memory. Furthermore we suggest a minimal characterization of the preparation device in order to lower the requirements for establishing a secure key.

==> Append.tex <==
\appendix
\section*{Appendix}
\subsection*{(i)}
W.l.o.g. we can consider Eve's projective measurements to be, 
\begin{eqnarray}
&& |M_e^{E=0}\rangle=\cos\frac{\alpha_e}{2}|0\rangle+\sin\frac{\alpha_e}{2}|1\rangle \nonumber \\
&& |M_e^{E=1}\rangle = |M_e^{E=0}\rangle^\perp \label{a4},
\end{eqnarray}
and $M_e^{E=0}=|M_e^{E=0}\rangle \langle M_e^{E=0} |$,$M_e^{E=0}=|M_e^{E=1}\rangle \langle M_e^{E=1}|$. Now one can rewrite (\ref{max2}) as,
\be \label{coolway!}
P_E^{max}(\eta) = \frac{1}{2}\max\left\{P_E^{a_0=a_1} + P_E^{a_0\neq a_1}(\eta) \right\},
\ee
where
\begin{equation} \label{subset1}
\begin{split}
P_E^{a_0 = a_1}=&
\frac{1}{4} Tr\bigg(\rho_{000}M^0_0 + \rho_{001}M^0_1 + \\
& \rho_{110}M^1_0 + \rho_{111}M^1_1\bigg), \\ 
\end{split}
\end{equation}
\begin{equation} \label{subset2}
\begin{split}
P_E^{a_0 \neq a_1}(\eta)= & \frac{1}{4} Tr\bigg(\rho_{010}\frac{M^0_0+\eta M^1_0}{1+\eta} + \\ & \rho_{011}\frac{M^1_1+\eta M^0_1}{1+\eta} + \rho_{100}\frac{M^1_0+\eta M^0_0}{1+\eta} + \\ & \rho_{101}\frac{M^1_1+\eta M^0_1}{1+\eta}\bigg.).
\end{split}
\end{equation}
Notice that (\ref{subset1}) and (\ref{subset2}) divide Alice's preparations into two mutually exclusive subsets. Alice's states that maximize $P_E^{a_0=a_1}$, $\rho_{0,0,0},\rho_{0,0,1},\rho_{1,1,0},\rho_{1,1,1}$ remain the same irrespective of whether Eve was able to correctly guess Bob's input ($e=b$) or not ($e\neq b$) simply because both of Alice's input are the same. This allows Eve to set these states equivalent to the projectors $M_0^0,M_1^0,M_0^1,M_1^1,$ respectively.   Which in-turn allows one to re-write (\ref{coolway!}) as,
\begin{equation}
\begin{split} \label{labelme}
P_E^{max}(\eta) = \frac{1}{2}(1+\max\{P_E^{a_0\neq a_1}(\eta)).
\end{split}
\end{equation}
Now in-order to find the maximum value of (\ref{subset2}) consider one of the terms involved,
\begin{equation}
\begin{split}
Tr\bigg(\rho_{010}\frac{M_0^0 + \eta M_0^1}{1+\eta}\bigg) = \frac{1}{1+\eta} - \frac{1-\eta}{1+\eta}Tr\bigg(\rho_{010}M_0^1\bigg),
\end{split}
\end{equation}
where the equality stems from the fact that $M_0^0=\mathbb{I}-M_0^1$.
The maximum for this term is reached by setting $\rho_{010}=M_0^0$ which yields the final security condition (\ref{maxMe}).
\subsection*{(ii)}
W.l.o.g she fixes Alice's preparations to be MUBs,
\begin{eqnarray}
&& \rho_{00}=|0\rangle\langle0|, \nonumber \\
&& \rho_{01}=\frac{1}{2}(|0\rangle+|1\rangle)(\langle0|+\langle1|), \nonumber \\
&& \rho_{10}=\frac{1}{2}(|0\rangle-|1\rangle)(\langle0|-\langle1|), \nonumber \\
&& \rho_{11}=|1\rangle\langle 1|, \label{c}
\end{eqnarray}
which is an optimal set of states for the standard ($2\to1$) QRAC \cite{Am2}. Next w.l.o.g. we characterize Eve's projective measurement using vectors from the same plane as the states in (\ref{c}),
\begin{eqnarray}
&& |M_e^{E=0}\rangle=\cos\frac{\alpha_e}{2}|0\rangle+\sin\frac{\alpha_e}{2}|1\rangle, \nonumber \\
&& |M_e^{E=1}\rangle = |M_e^{E=0}\rangle^\perp \label{a4},
\end{eqnarray}
and $M_e^{E}=|M_e^E\rangle\langle M_e^E|$. This allows us to partition (\ref{max2}) into two parts based on different values of $e$. These parts are independent and, due to symmetry, equal. Therefore we may re-write $P_E(\eta)$ as ,
\be
P_E(\eta)=\max\left\{\frac{P_{E_0}^0+\eta P_{E_1}^0}{1+\eta}\right\},
\ee 
which is,
\begin{equation}
\begin{split}
P_E(\eta)= &
\frac{1}{8(1+\eta)}Tr\bigg(M_{e=0}^{E=0}(\rho_{00}+\rho_{01})+ \\ & M_{e=0}^{E=1}(\rho_{10}+\rho_{11})\bigg)
+ \\& \frac{\eta}{8(1+\eta)} Tr\bigg(M_{e=0}^{E=0}(\rho_{00}+\rho_{10})+ \\ & M_{e=0}^{E=1}(\rho_{01}+\rho_{11})\bigg).
\end{split}
\end{equation}
After plugging in (\ref{c}),(\ref{a4}), this yields,
\begin{equation}
\begin{split}
P_E^{max}(\eta)& =\max_{\alpha_0}(P_E(\eta)) \\ & = \frac{1}{4}\left(2+\cos \alpha_0+\frac{1-\eta}{1+\eta}\sin\alpha_0\right).
\end{split}
\end{equation}
This expression is maximized for $\alpha_\eta=\arctan\left(\frac{1-\eta}{1+\eta}\right)$. Hence, we obtain the security condition (\ref{m1}).
\subsection*{(iii)}
Here the success probability for Eve is,
\begin{equation}
P_E(\eta)= \frac{1}{8(1+\eta)}Tr \sum_{a_0a_1eb} \eta^{1-\delta_{eb}}P(E=a_b|a_0,a_1,e,b),
\end{equation}
which can in-turn be expressed as,
\begin{equation}
\begin{split}
P_E(\eta)= \frac{1}{8} Tr\bigg[ & \sum_{i,j} \tilde{\rho}_{i,i,j} \frac{M_{i,i}^{E=j} \otimes \mathbb{I} + \eta M_{i,1-i}^{E=j} \otimes \mathbb{I} }{1 + \eta} + \\ & \tilde{\rho}_{i,1-i,j} \frac{M_{i,i}^{E=1-\delta_{i,j}} \otimes \mathbb{I} + \eta M_{i,1-i}^{E=\delta_{i,j}} \otimes \mathbb{I} }{1 + \eta} \bigg].
\end{split}
\end{equation}
Notice that this expression constitutes four independent elements  for specific value of the pair $(i,j)$. In order to find $P_E(\eta)^{max}$ we need only find the maximizing condition for one term. Let's consider a particular pair $(i,j)$, then the expression for $P_E(\eta)^{max}$ simplifies to,
\begin{equation}
\begin{split}
P_E^{max}(\eta)= & \frac{1}{2} \max \bigg\{ Tr\bigg(  \tilde{\rho}_{i,i,j} \frac{M_{i,i}^{E=j} \otimes \mathbb{I} + \eta M_{i,1-i}^{E=j} \otimes \mathbb{I} }{1 + \eta} + \\ & \tilde{\rho}_{i,1-i,j} \frac{M_{i,i}^{E=1-\delta_{i,j}} \otimes \mathbb{I} + \eta M_{i,1-i}^{E=\delta_{i,j}} \otimes \mathbb{I} }{1 + \eta} \bigg) \bigg\}.
\end{split}
\end{equation}
This equation is maximized when $M_{i,i}^{E=j}=M_{i,1-i}^{E=j}$ or $M_{i,i}^{E=1-\delta_{i,j}}=M_{i,1-i}^{E=\delta_{i,j}}$ yielding the same security condition as (\ref{maxMe}).
\subsection*{(iv)}
In the case when Eve does not have access to quantum memory (IR) we can re-write (\ref{max3}) in a convenient way as,
\begin{equation}
P_E^{max}(\eta)=\frac{1}{4}\max \bigg\{P_E^{a_0=a_1=a_2} + P_E^{NOT\{a_0=a_1=a_2\}} \bigg\},
\end{equation}
where $P_E^{a_0=a_1=a_2}$ is Eve's success probability for the case when all three of the input bits of Alice are equal and $P_E^{NOT\{a_0=a_1=a_2\} }$ is Eve's success probability for the case when the three inputs of Alice are not equal. As Alice's states and Bob's measurement that maximize $P_E^{a_0=a_1=a_2}$ remain the same irrespective of the fact whether Eve was able to guess Bob's input correctly or not we can further re-write this as,
\begin{equation}
P_E^{max}(\eta)=\frac{1}{4}\bigg( 1 + \max \bigg\{P_E^{NOT\{a_0=a_1=a_2\}} \bigg\} \bigg).
\end{equation}
Following exactly the same steps as above this yields the security condition (\ref{3to1max}).
\subsection*{(v)}
We find that the optimal states are,
\begin{eqnarray}
&& |000\rangle=|0\rangle,\nonumber\\
&& |001\rangle=\cos \frac{\alpha}{2}|0\rangle+\sin\frac{\alpha}{2}|1\rangle,\nonumber\\
&& |010\rangle=\cos \frac{\alpha}{2}|0\rangle+e^{i\beta}\sin\frac{\alpha}{2}|1\rangle,\nonumber\\
&& |100\rangle=\cos \frac{\alpha}{2}|0\rangle+e^{-i\beta}\sin\frac{\alpha}{2}|1\rangle,\nonumber\\
&& |111\rangle=|000\rangle^\perp ,\nonumber \\
&& |110\rangle=|001\rangle^\perp ,\nonumber \\
&& |101\rangle=|010\rangle^\perp ,\nonumber \\
&& |011\rangle=|100\rangle^\perp,\label{a11}
\end{eqnarray}
where $\alpha$ and $\beta$ are parameters controlled by Eve.  In this case optimal encoding for standard $(3\to1)$ QRAC is reproduced for $\alpha=\arccos\frac{1}{3}$ and $\beta=2\pi/3$.
For Eve's measurements ($ M_e^{E=a_b}=|M_e^{E=a_b}\rangle\langle M_e^{E=a_b}|$) we use the following parametrization
\begin{eqnarray}
&& |M_e^{E=0}\rangle = \cos\frac{\alpha_e}{2}|0\rangle+e^{i\beta_e}\sin\frac{\alpha_e}{2}|1\rangle \nonumber \\
&& |M_e^{E=1}\rangle = |M_e^{E=0}\rangle^\perp \label{a2},
\end{eqnarray} 
A straightforward maximization yields the security condition (\ref{max3to1res}).
